Physics Informed Neural Network Framework for Unsteady Discretized Reduced Order System

This work addresses the development of a physics-informed neural network (PINN) with a loss term derived from a discretized time-dependent reduced-order system. In this work, first, the governing equations are discretized using a finite difference scheme (whereas, any other discretization technique can be adopted), then projected on a reduced or latent space using the Proper Orthogonal Decomposition (POD)-Galerkin approach and next, the residual arising from discretized reduced order equation is considered as an additional loss penalty term alongside the data-driven loss term using different variants of deep learning method such as Artificial neural network (ANN), Long Short-Term Memory based neural network (LSTM). The LSTM neural network has been proven to be very effective for time-dependent problems in a purely data-driven environment. The current work demonstrates the LSTM network's potential over ANN networks in physics-informed neural networks (PINN) as well. The potential of using discretized governing equations instead of continuous form lies in the flexibility of input to the PINN. Different sizes of data ranging from small, medium to big datasets are used to assess the potential of discretized-physics-informed neural networks when there is very sparse or no data available. The proposed methods are applied to a pitch-plunge airfoil motion governed by rigid-body dynamics and a one-dimensional viscous Burgers' equation. The current work also demonstrates the prediction capability of various discretized-physics-informed neural networks outside the domain where the data is available or governing equation-based residuals are minimized.

==> Command.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\def\a{{\bm a}}
\def\b{{\bm b}}
\def\d{{\bm d}}
\def\f{{\bm f}}
\def\g{{\bm g}}
\def\n{{\bm n}}
\def\u{{\bm u}}
\def\v{{\bm v}}
\def\w{{\bm w}}
\def\x{{\bm x}}
\def\P{{\bm P}}
\def\U{{\bm U}}
\def\X{{\bm X}}
\def\0{\boldsymbol{0}}
\def\ss{\boldsymbol{\sigma}}
\def\SS{\boldsymbol{\Sigma}}
\def\ee{\boldsymbol{\eta}}
\def\mubar{\overline{\mu}}
\def\ubar{\overline{\u}}
\def\vbar{\overline{\v}}
\def\vtilde{\tilde{\v}}
\def\wbar{\overline{\w}}
\def\qbar{\overline{q}}
\def\dt{\partial_t}
\def\bbf{\mathbf{b}}
\def\ebf{\mathbf{e}}
\def\fbf{\mathbf{f}}
\def\qbf{\mathbf{q}}
\def\pbf{\mathbf{p}}
\def\vbf{\mathbf{v}}
\def\ubf{\mathbf{u}}
\def\xbf{\mathbf{x}}
\def\ybf{\mathbf{y}}
\def\vbarbf{\overline{\vbf}}
\def\qbarbf{\overline{\qbf}}
\def\xbarbf{\overline{\xbf}}
\def\bbarbf{\overline{\bbf}}

\def\uh{\u_h}
\def\vh{\v_h}
\def\fh{\f_h}
\def\bh{\b_h}
\def\ph{p_h}
\def\qh{q_h}
\def\vbarh{\vbar_h}
\def\qbarh{\qbar_h}
\def\mubarh{\mubar_h}

\def\cl {\nonumber \\}
\def\el {\nonumber }

\newtheorem{rem}{Remark}[section]

\def\Jcp{J. Comp. Phys}
\def\Cmame{Comput. Methods Appl. Mech. Engrg.}
\def\Jmpa{J. Math. Pures Appl.}
\def\Mmmas{Math. Model Meth. Appl. Sci.}
\def\Siamsc{SIAM J. Sci. Comp.}

\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\def\div{\nabla\cdot}
\def\grad{\nabla}
\def\grads{\grad^s}

%\topmargin      10mm 
%\evensidemargin 5mm \oddsidemargin  5mm
%\textwidth      150mm \textheight 200mm \frenchspacing \sloppy

%\def\baselinestretch{2} 

\newcommand{\anna}[2][cyan]{\emph{\textcolor{#1}{#2}}}
\newcommand{\rev}[2][red]{{\textcolor{#1}{#2}}}



% To quantify the ROM accuracy, all snapshots are reconstructed in time using ROM techniques and the $l^2$-norm relative error for each snapshot is computed considering again three different energy threshold as before.  We were interested to see the effect of Dataset Size, i.e. Train to Test Split Ratios in our comparison to check the error convergence with the respect to this ratio. To this aim three ratio were considered; in the first case 50$\%$ of dataset is used to train the model, then 70$\%$ and finally 90$\%$ each of them for three various energy threshold.     
